Anti-clustering in the national SARS-CoV-2 daily infection counts

The noise in daily infection counts of an epidemic should be super-Poissonian due to intrinsic epidemiological and administrative clustering. Here, we use this clustering to classify the official national SARS-CoV-2 daily infection counts and check for infection counts that are unusually anti-clustered. We adopt a one-parameter model of $\phi'_i$ infections per cluster, dividing any daily count $n_i$ into $n_i/\phi'_i$ 'clusters', for 'country' $i$. We assume that $n_i/\phi'_i$ on a given day $j$ is drawn from a Poisson distribution whose mean is robustly estimated from the four neighbouring days, and calculate the inferred Poisson probability $P'_{ij}$ of the observation. The $P'_{ij}$ values should be uniformly distributed. We find the value $\phi_i$ that minimises the Kolmogorov-Smirnov distance from a uniform distribution. We investigate the $(\phi_i, N_i)$ distribution, for total infection count $N_i$. We find that most of the daily infection count sequences are inconsistent with a Poissonian model. Most are found to be consistent with the $\phi_i$ model. The 28-, 14- and 7-day least noisy sequences for several countries are best modelled as sub-Poissonian, suggesting a distinct epidemiological family. The 28-day least noisy sequence of Algeria has a preferred model that is strongly sub-Poissonian, with $\phi_i^{28} < 0.1$. TJ, TR, RU, BY, AL, AE, and NI have preferred models that are also sub-Poissonian, with $\phi_i^{28} < 0.5$. A statistically significant ($P^{\tau} < 0.05$) correlation was found between the lack of media freedom in a country, as represented by a high Reporters sans frontieres Press Freedom Index (PFI$^{2020}$), and the lack of statistical noise in the country's daily counts. The $\phi_i$ model appears to be an effective detector of suspiciously low statistical noise in the national SARS-CoV-2 daily infection counts.

==> AIC_BIC_full.tex <==
\rule{0ex}{2.6ex}%
 & 268.60 & 848.87 & 289.91 & 870.18 & 377.52 & 957.79 & 313.21 & 878.50 & 208.49 & 743.75 \\
\hline


==> AIC_BIC_full_jhu.tex <==
\rule{0ex}{2.6ex}%
 & 376.18 & 994.94 & 401.69 & 1020.44 & 498.00 & 1116.75 & 421.96 & 1032.94 & 239.83 & 811.89 \\
\hline


==> Makefile <==
paper.pdf: paper-full.tex
	latex paper-full && latex paper-full && latex paper-full \n	&&dvips paper-full -o paper-tmp.eps \n	&&ps2pdf paper-tmp.eps \n	&&mv -v paper.pdf subpoisson.pdf

.PHONY: clean
clean:
	rm -f *.aux *.auxlock *.bbl *.bcf
	rm -f *.blg *.log *.out *.run.xml


==> low_phi_table_07days.tex <==
\rule{0ex}{2.6ex}%
United~Arab~Emirates & 207822 & 544.9 & 0.24 & 0.99 & 0.05 & 2020-04-27 \\
India & 10266674 & 10109.3 & 0.34 & 0.60 & 0.05 & 2020-06-06 \\
Turkey & 2669568 & 929.6 & 0.22 & 0.93 & 0.05 & 2020-07-15 \\
Tajikistan & 13062 & 51.9 & 0.16 & 0.77 & 0.05 & 2020-06-28 \\
Albania & 58316 & 297.7 & 0.23 & 0.98 & 0.05 & 2020-10-18 \\
Belarus & 194284 & 947.9 & 0.60 & 0.94 & 0.05 & 2020-05-13 \\
Algeria & 99610 & 204.3 & 0.37 & 0.49 & 0.05 & 2020-10-14 \\
Russia & 3159297 & 5076.7 & 0.36 & 0.68 & 0.10 & 2020-08-09 \\
Ethiopia & 124264 & 456.7 & 0.83 & 0.93 & 0.13 & 2020-12-13 \\
Poland & 1294878 & 297.7 & 0.31 & 0.96 & 0.16 & 2020-06-20 \\
\hline


==> low_phi_table_07days_jhu.tex <==
\rule{0ex}{2.6ex}%
United~Arab~Emirates & 529220 & 544.9 & 0.24 & 0.99 & 0.05 & 2020-04-27 \\
Turkey & 4955594 & 929.6 & 0.22 & 0.93 & 0.05 & 2020-07-15 \\
Albania & 131419 & 297.7 & 0.23 & 0.98 & 0.05 & 2020-10-18 \\
Belarus & 363732 & 947.9 & 0.60 & 0.94 & 0.05 & 2020-05-13 \\
Algeria & 123272 & 204.3 & 0.37 & 0.49 & 0.05 & 2020-10-14 \\
Russia & 4792354 & 5035.0 & 0.38 & 0.75 & 0.10 & 2020-08-09 \\
Poland & 2811951 & 297.0 & 0.51 & 0.99 & 0.10 & 2020-06-20 \\
Saudi~Arabia & 422316 & 175.6 & 0.52 & 0.99 & 0.15 & 2021-01-13 \\
Syria & 23121 & 82.3 & 0.21 & 0.97 & 0.17 & 2020-08-14 \\
Panama & 365975 & 171.1 & 0.82 & 0.96 & 0.17 & 2020-05-09 \\
\hline


==> low_phi_table_14days.tex <==
\rule{0ex}{2.6ex}%
Algeria & 99610 & 285.9 & 0.12 & 0.40 & 0.05 & 2020-09-01 \\
Nicaragua & 6046 & 73.6 & 0.12 & 0.98 & 0.08 & 2020-09-22 \\
Tajikistan & 13062 & 64.6 & 0.02 & 0.99 & 0.09 & 2020-06-11 \\
United~Arab~Emirates & 207822 & 521.2 & 0.11 & 0.56 & 0.09 & 2020-04-19 \\
Turkey & 2669568 & 971.6 & 0.12 & 0.86 & 0.11 & 2020-07-08 \\
Belarus & 194284 & 945.6 & 0.22 & 1.00 & 0.13 & 2020-05-12 \\
Albania & 58316 & 143.4 & 0.21 & 0.96 & 0.17 & 2020-09-01 \\
Russia & 3159297 & 5627.0 & 0.47 & 0.98 & 0.20 & 2020-07-21 \\
Saudi~Arabia & 331359 & 1227.5 & 0.38 & 0.96 & 0.30 & 2020-04-19 \\
Syria & 4931 & 76.6 & 0.42 & 0.96 & 0.35 & 2020-08-14 \\
\hline


==> low_phi_table_14days_jhu.tex <==
\rule{0ex}{2.6ex}%
United~Arab~Emirates & 529220 & 3384.1 & 0.07 & 0.35 & 0.05 & 2021-01-11 \\
Algeria & 123272 & 336.4 & 0.06 & 0.80 & 0.05 & 2020-08-26 \\
Turkey & 4955594 & 971.6 & 0.12 & 0.86 & 0.11 & 2020-07-08 \\
Belarus & 363732 & 945.6 & 0.22 & 1.00 & 0.13 & 2020-05-12 \\
Albania & 131419 & 143.4 & 0.16 & 0.92 & 0.15 & 2020-09-01 \\
Saudi~Arabia & 422316 & 337.7 & 0.32 & 0.79 & 0.20 & 2021-02-08 \\
Russia & 4792354 & 5165.5 & 0.47 & 0.51 & 0.28 & 2020-08-01 \\
Syria & 23121 & 76.6 & 0.42 & 0.96 & 0.35 & 2020-08-14 \\
Poland & 2811951 & 299.9 & 0.55 & 0.68 & 0.53 & 2020-06-17 \\
Kenya & 161393 & 126.2 & 0.54 & 0.91 & 0.57 & 2020-06-03 \\
\hline


==> low_phi_table_28days.tex <==
\rule{0ex}{2.6ex}%
Algeria & 99610 & 227.6 & 0.00 & 0.36 & 0.05 & 2020-09-03 \\
Tajikistan & 13062 & 63.0 & 0.02 & 0.96 & 0.13 & 2020-06-07 \\
Turkey & 2669568 & 1014.5 & 0.03 & 1.00 & 0.14 & 2020-06-30 \\
Russia & 3159297 & 5403.8 & 0.26 & 0.59 & 0.20 & 2020-07-20 \\
Belarus & 194284 & 921.9 & 0.14 & 0.89 & 0.21 & 2020-05-08 \\
Albania & 58316 & 203.8 & 0.33 & 0.64 & 0.23 & 2020-09-27 \\
United~Arab~Emirates & 207822 & 512.8 & 0.08 & 0.23 & 0.23 & 2020-04-14 \\
Nicaragua & 6046 & 135.7 & 0.17 & 0.77 & 0.30 & 2020-07-07 \\
Syria & 4931 & 70.0 & 0.19 & 0.91 & 0.50 & 2020-08-15 \\
Saudi~Arabia & 331359 & 1182.2 & 0.47 & 0.54 & 1.11 & 2020-04-12 \\
\hline


==> low_phi_table_28days_jhu.tex <==
\rule{0ex}{2.6ex}%
Algeria & 123272 & 338.2 & 0.02 & 0.72 & 0.05 & 2020-08-18 \\
Turkey & 4955594 & 1014.5 & 0.03 & 1.00 & 0.14 & 2020-06-30 \\
United~Arab~Emirates & 529220 & 2884.9 & 0.01 & 0.07 & 0.15 & 2020-12-30 \\
Belarus & 363732 & 921.9 & 0.14 & 0.89 & 0.21 & 2020-05-08 \\
Albania & 131419 & 203.8 & 0.33 & 0.64 & 0.23 & 2020-09-27 \\
Russia & 4792354 & 5414.0 & 0.36 & 0.85 & 0.24 & 2020-07-19 \\
Saudi~Arabia & 422316 & 332.5 & 0.54 & 0.78 & 0.43 & 2021-02-01 \\
Syria & 23121 & 70.0 & 0.19 & 0.91 & 0.50 & 2020-08-15 \\
Iran & 2591609 & 6594.5 & 0.14 & 0.41 & 1.51 & 2021-01-15 \\
Georgia & 315913 & 384.4 & 0.79 & 0.99 & 1.66 & 2020-09-17 \\
\hline


==> low_phi_table_full.tex <==
\rule{0ex}{2.6ex}%
Nicaragua & 6046 & 0.17 & 0.77 & 0.30 & 0.003 & 0.66 & 0.30 & 0.17 & 0.00 \\
Syria & 4931 & 0.29 & 0.92 & 0.58 & 0.008 & 0.92 & 0.58 & 0.29 & 0.00 \\
Tajikistan & 13062 & 0.17 & 0.76 & 0.63 & 0.005 & 0.78 & 0.67 & 0.16 & 0.00 \\
Algeria & 99610 & 0.01 & 0.17 & 0.65 & 0.002 & 0.13 & 0.62 & 0.01 & 0.00 \\
Belarus & 194284 & 0.01 & 0.53 & 1.70 & 0.003 & 0.40 & 1.57 & 0.46 & 0.58 \\
Croatia & 210837 & 0.27 & 0.89 & 3.24 & 0.007 & 0.89 & 3.24 & 0.70 & 1.02 \\
Albania & 58316 & 0.00 & 0.44 & 3.27 & 0.013 & 0.41 & 3.27 & 0.30 & 1.80 \\
New~Zealand & 2164 & 0.44 & 0.90 & 4.32 & 0.092 & 0.94 & 4.32 & 0.86 & 1.19 \\
Australia & 28430 & 0.11 & 0.90 & 5.07 & 0.030 & 0.90 & 5.69 & 0.87 & 3.55 \\
Thailand & 6884 & 0.29 & 0.99 & 5.37 & 0.064 & 0.99 & 5.37 & 0.96 & 3.80 \\
\hline\rule{0ex}{2.6ex}%
Algeria & 99610 & 0.01 & 0.17 & 0.65 & 0.002 & 0.13 & 0.62 & 0.01 & 0.00 \\
Belarus & 194284 & 0.01 & 0.53 & 1.70 & 0.003 & 0.40 & 1.57 & 0.46 & 0.58 \\
Nicaragua & 6046 & 0.17 & 0.77 & 0.30 & 0.003 & 0.66 & 0.30 & 0.17 & 0.00 \\
Turkey & 2669568 & 0.00 & 0.20 & 6.46 & 0.003 & 0.16 & 6.09 & 0.16 & 5.07 \\
Russia & 3159297 & 0.00 & 0.24 & 7.24 & 0.004 & 0.19 & 7.08 & 0.22 & 6.03 \\
Tajikistan & 13062 & 0.17 & 0.76 & 0.63 & 0.005 & 0.78 & 0.67 & 0.16 & 0.00 \\
Croatia & 210837 & 0.27 & 0.89 & 3.24 & 0.007 & 0.89 & 3.24 & 0.70 & 1.02 \\
Syria & 4931 & 0.29 & 0.92 & 0.58 & 0.008 & 0.92 & 0.58 & 0.29 & 0.00 \\
Saudi~Arabia & 331359 & 0.00 & 0.91 & 6.31 & 0.010 & 0.84 & 6.17 & 0.83 & 4.90 \\
Iran & 1225142 & 0.00 & 0.82 & 12.73 & 0.011 & 0.58 & 11.61 & 0.71 & 11.35 \\
\hline


==> low_phi_table_full_jhu.tex <==
\rule{0ex}{2.6ex}%
Syria & 23121 & 0.48 & 0.94 & 0.72 & 0.004 & 0.94 & 0.72 & 0.48 & 0.00 \\
Algeria & 123272 & 0.04 & 0.19 & 0.98 & 0.002 & 0.20 & 1.00 & 0.04 & 0.00 \\
Croatia & 339412 & 0.27 & 0.89 & 3.24 & 0.005 & 0.89 & 3.24 & 0.70 & 1.02 \\
Saudi~Arabia & 422316 & 0.00 & 0.83 & 3.67 & 0.005 & 0.66 & 3.55 & 0.62 & 2.43 \\
New~Zealand & 2637 & 0.10 & 0.88 & 3.85 & 0.074 & 0.89 & 4.68 & 0.90 & 3.63 \\
Albania & 131419 & 0.00 & 0.16 & 4.90 & 0.013 & 0.17 & 4.90 & 0.09 & 3.76 \\
Thailand & 74921 & 0.29 & 0.99 & 5.37 & 0.019 & 0.99 & 5.37 & 0.96 & 3.80 \\
Denmark & 257182 & 0.00 & 0.97 & 5.56 & 0.010 & 0.99 & 5.56 & 0.91 & 5.50 \\
Iceland & 6498 & 0.33 & 1.00 & 5.96 & 0.073 & 0.99 & 5.96 & 0.95 & 4.27 \\
Greece & 352027 & 0.03 & 0.98 & 6.53 & 0.011 & 0.92 & 5.43 & 0.67 & 5.50 \\
\hline\rule{0ex}{2.6ex}%
Algeria & 123272 & 0.04 & 0.19 & 0.98 & 0.002 & 0.20 & 1.00 & 0.04 & 0.00 \\
Russia & 4792354 & 0.00 & 0.31 & 10.12 & 0.004 & 0.26 & 9.44 & 0.26 & 8.81 \\
Syria & 23121 & 0.48 & 0.94 & 0.72 & 0.004 & 0.94 & 0.72 & 0.48 & 0.00 \\
Croatia & 339412 & 0.27 & 0.89 & 3.24 & 0.005 & 0.89 & 3.24 & 0.70 & 1.02 \\
Saudi~Arabia & 422316 & 0.00 & 0.83 & 3.67 & 0.005 & 0.66 & 3.55 & 0.62 & 2.43 \\
Iran & 2591609 & 0.00 & 0.33 & 11.61 & 0.007 & 0.17 & 10.00 & 0.25 & 9.66 \\
Turkey & 4955594 & 0.00 & 0.02 & 19.95 & 0.008 & 0.01 & 19.27 & 0.01 & 16.98 \\
Denmark & 257182 & 0.00 & 0.97 & 5.56 & 0.010 & 0.99 & 5.56 & 0.91 & 5.50 \\
Hungary & 785967 & 0.02 & 0.99 & 9.23 & 0.010 & 0.98 & 14.29 & 0.91 & 7.00 \\
Belarus & 363732 & 0.00 & 0.01 & 6.92 & 0.011 & 0.01 & 6.46 & 0.01 & 5.13 \\
\hline


==> pfi_correlations_table.tex <==
\rule{0ex}{2.6ex}%
$\phi_i$ & -0.118 & 0.131 & -0.126 & 0.108 & -0.148 & 0.0584 & -0.200 & 0.0108  \\
$\psi_i$ & -0.160 & 0.0408 & -0.157 & 0.0445 & -0.176 & 0.0249 & -0.170 & 0.0300  \\
\hline


==> pfi_correlations_table_jhu.tex <==
\rule{0ex}{2.6ex}%
$\phi_i$ & -0.124 & 0.105 & -0.158 & 0.0400 & -0.175 & 0.0230 & -0.232 & 0.00254  \\
$\psi_i$ & -0.165 & 0.0318 & -0.162 & 0.0346 & -0.163 & 0.0339 & -0.194 & 0.0112  \\
\hline

